Statistical Guarantees for Approximate Stationary Points of Shallow Neural Networks

Since statistical guarantees for neural networks are usually restricted to global optima of intricate objective functions, it is unclear whether these theories explain the performances of actual outputs of neural network pipelines. The goal of this paper is, therefore, to bring statistical theory closer to practice. We develop statistical guarantees for shallow linear neural networks that coincide up to logarithmic factors with the global optima but apply to stationary points and the points nearby. These results support the common notion that neural networks do not necessarily need to be optimized globally from a mathematical perspective. We then extend our statistical guarantees to shallow ReLU neural networks, assuming the first layer weight matrices are nearly identical for the stationary network and the target. More generally, despite being limited to shallow neural networks for now, our theories make an important step forward in describing the practical properties of neural networks in mathematical terms.

==> Sections/Proof_The_1_high-level.tex <==

\begin{proof}
The proof approach is based on  Taylor's theorem,   the definition of stationary points, Lemma~\ref{EmpProcctwo}, and Proposition~\ref{PSDHessian}. 

	We start by writing a second-order Taylor expansion of  $\objectiveFP{\StarOutSc,\StarInSc}$ (the risk in a rescaled version of the target with $\ParamVSSc=\vectorize(\StarOutSc,\StarInSc)\in\R^{\EfDim}$) around a rescaled version of a reasonable stationary  $\ParamStaSc=\vectorize(\StaOutSc,\StaInSc)\in\R^{\EfDim}$ with suitable  $\Sc\in\R^{\nbrwidth}$ to get
\begin{linenomath}
	\begin{align*}
		\objectiveFP{\StarOutSc,\StarInSc}&=\objectiveFP{\StaOutSc,\StaInSc}+\DervPopG[\StaOutSc,\StaInSc]\tp(\ParamVSSc-\ParamStaSc)\\
		&~~~+\frac{1}{2}(\ParamVSSc-\ParamStaSc)\tp \HessianF{\StaOutSc+\TayPar(\StarOutSc-\StaOutSc),\StaInSc+\TayPar(\StarInSc-\StaInSc)}(\ParamVSSc-\ParamStaSc)
	\end{align*}
\end{linenomath}
for some $\TayPar\in(0,1)$~\citep[Proposition~1.1.13.a]{bertsekas2006convex}.
Employing the property of  rescaled networks, using the fact that $\DervPopG[\StaOutSc,\StaInScTr]\tp(\ParamVSScTr-\ParamStaScTr)=\DervPopG[\StaOut,\StaIn]\tp(\ParamVS-\ParamSta)$, and  shorthand notation 
\begin{linenomath}
	\begin{equation*}
		\SEigenV\deq(\ParamVSSc-\ParamStaSc)\tp \HessianF{\StaOutSc+\TayPar(\StarOutSc-\StaOutSc),\StaInSc+\TayPar(\StarInSc-\StaInSc)}(\ParamVSSc-\ParamStaSc)   
	\end{equation*}
\end{linenomath}
we obtain
 \begin{linenomath}
\begin{equation*}
    \objectiveFP{\parameteroutS,\parameterinS}=\objectiveFP{\StaOut,\StaIn}+\DervPopSta\tp(\ParamVS-\ParamSta)+\frac{1}{2}\SEigenV\,.
\end{equation*}
 \end{linenomath}
Also,  the definition of stationary points in~\eqref{StaP} and doing some machinery imply
 \begin{linenomath}
\begin{align*}
    \DervSamSta\tp(\ParamVS-\ParamSta)+\tuning\normone{\ParamVS}-\tuning\normone{\ParamSta}\ge 0\,.
\end{align*}
 \end{linenomath}
and 
 \begin{linenomath}
\begin{equation*}
   -\DervPopSta\tp(\ParamVS-\ParamSta)\le \bigl(\DervSamSta-\DervPopSta\bigr)\tp(\ParamVS-\ParamSta)+\tuning\normone{\ParamVS}-\tuning\normone{\ParamSta}\,.
\end{equation*}
 \end{linenomath}
Using our Taylor expansion together with inequality above  gives
 \begin{linenomath}
\begin{equation*}
  \objectiveFP{\StaOut,\StaIn}-\objectiveFP{\parameteroutS,\parameterinS}+\frac{1}{2}\SEigenV\le \bigl(\DervSamSta-\DervPopSta\bigr)\tp(\ParamVS-\ParamSta)+\tuning\normone{\ParamVS}-\tuning\normone{\ParamSta}\,.
\end{equation*}
 \end{linenomath}
Rearranging and employing our Lemma~\ref{EmpProcctwo} gives 
 \begin{linenomath}
\begingroup
\allowdisplaybreaks
\begin{align*}
  \objectiveFP{\StaOut,\StaIn}
   &\le  \objectiveFP{\parameteroutS,\parameterinS}+2\tuning\normone{\ParamVS}+\tuningopt \normone{\ParamVS-\ParamSta}+\frac{\tuningopt}{2\nbrsamples}-\tuning\normone{\ParamVS-\ParamSta}-\frac{1}{2}\SEigenV
\end{align*}
\endgroup
 \end{linenomath}
with probability at least   $1-1/2\nbrsamples$.


The third and fifth terms in the last inequality above  can be canceled if we choose the tuning parameter large enough. Hence, for $\tuning\ge \tuningopt$ we obtain
 \begin{linenomath}
\begin{equation*}
  \objectiveFP{\StaOut,\StaIn}
    \le \objectiveFP{\parameteroutS,\parameterinS}+2\tuning\normone{\ParamVS}+\frac{\tuningopt}{2\nbrsamples}-\frac{1}{2}\SEigenV\,.
\end{equation*}
 \end{linenomath}


The rest of the proof is analysing the behavior of $\SEigenV$ using 
Proposition~\ref{PSDHessian} that leaves us with $\SEigenV~\in(0,\infty)$, as desired (for simplicity we assume here that the corresponding line-segment is an invertible matrix; see our detailed proof in Supplementary~\ref{proofs} how we relax this assumption in general). 
\end{proof}


==> Sections/body.tex <==
\section{Introduction}
Statistical theories for deep learning usually apply to exact, global optima of certain objective functions \citep{Bartlett1998,bauer2019deep,kohler2021rate,2021LedererSparse,schmidt2020,mohades2023reducing,golestanehmany}.
But those objective functions cannot be solved explicitly and are highly non-convex,
so that in practice, exact, global optimization is---at least to date---an open research question, 
	and we can currently expect only approximate stationary points from current (general) algorithms (see Figure~\ref{fig:minima}).
In other words,
it is unclear whether the known theories have any meaning for the outputs of actual deep-learning pipelines.

\figureminima

Also other parts of machine learning face optimization problems that are challenging to optimize globally and to full precision.
Accordingly, some statistical insights have already been established.
For example,
\citet{bien2018non,bien2019prediction} solve a non-convex problem in linear regression in a ``convex'' way and develop statistical theories for their solution.
Some insights on the statistical theory of stationary points for (simple) non-convex objectives have already been presented:
	\citet[Theorems~1,2]{loh2015} extract statistical guarantees for stationary points of  non-convex objectives (allowing for non-convexity in both loss and penalty functions) in a regression-type settings, under a  so-called  ``restricted-strong convexity" condition over the empirical loss (see their Display (4)).
	\citet[Theorem~1]{loh2017statistical} studies the behavior of stationary points of penalized robust estimators in a linear-regression setting. 
	They prove that under a local ``restricted-strong convexity"  condition, stationary points within the region of restricted curvature are  statistically consistent with the target.
	Also~\citet[Theorem~1]{elsener2018sharp} derive sharp oracle inequalities for stationary points of  general non-convex objectives  made by a non-convex loss plus a convex penalty, under a  restrictive condition called  ``two point marginal  condition" on the theoretical loss.
	They exemplify their bounds for  simple models like robust regression and binary classification.
	Their condition is kinda similar to the restricted-strong convexity but on the theoretical loss (and not on the empirical loss). 
%	Unfortunately,
%	the curvature assumptions in these papers are infeasible for neural network settings, which means that their approaches cannot be applied here.
	 
%\citet{loh2015} and \citet{loh2017statistical} develop statistical theory for stationary points in another regression setup under curvature assumptions.
%\citet{elsener2018sharp} establish more general theories for stationary points also under curvature assumptions.
%\citet{Taheri2019} propose an algorithm and statistical theory for approximate solutions in a convex setting.
%But it is currently unclear how to extend these insights to deep learning---if at all possible.
However, it remains unclear how to extend these insights to deep learning, as they either apply only to simple models like linear regression or rely on specific curvature assumptions, while it is not clear if such curvature properties hold even for simple networks.

This paper develops statistical guarantees for the  stationary points of shallow neural networks  and for the points in the vicinity of them.
Strikingly, our statistical rates match the  rates of global optimizers up to log-terms \citep{taheri2021,2021LedererSparse,golestanehmany}.
Thus, our results establish a mathematical proof of the ``empirical fact'' that global optimization is not necessary in deep learning.
This complements and contrasts studies about the existence or non-existence of spurious local minima and saddle points in both linear and non-linear networks~\citep{zhou2018critical,fukumizu2000local,safran2018spurious,lederer2020no,liu2022spurious}.
%Although our theories here are limited to shallow networks, our paper makes a significant step toward the mathematical understanding of practical neural-network pipelines.

One of the main challenges in the proofs is the complexity, intricacy, and ambiguity of the parameter space of neural networks.
To  address this challenge,
we introduce scaling tricks~\citep{taheri2021} and use particular arguments from empirical-process theory for regularized objectives.
Moreover, in strong contrast to most theory papers,
we focus on regression,
which is more general and mathematically more challenging than classification. 
For example, unbounded losses like least-squares cannot be treated (at least not directly) with standard techniques like McDiarmid's inequality~\citep[Lemma~3.3]{mcdiarmid1989method} or Rademacher complexities~\citep[Chapter~3]{mohri2018foundations}. 
Thus, our work also contributes considerably on the technical aspects of deep learning.

%\Res{Also,  most of the theory and applied deep learning papers  focus on classification setting, 
	%while the regression setting is much more challenging.
	%Unbounded loss  makes regular techniques like McDiarmid's inequality~\citep[Lemma~3.3]{mcdiarmid1989method} not applicable for regression settings. 
	%So, our empirical processes approach seems more general and can also be employed for classification. 
	%}
%\Res{We employ the tools from empirical process theory for choosing a suitable tuning parameter for regularized neural networks. 
	%While interesting, employing this technique is not straightforward especially for neural networks;
	%main challenge is computing the complexity of parameter space efficiently, in this case neural networks. 
	% }



%\paragraph{Motivation}
%Let us briefly motivate our study in a very simple example.
%Consider regression data consisting of the two input-output pairs $(\datainE_1,\dataoutE_1)=(-1,0)$ and  $(\datainE_2,\dataoutE_2)=(1,1)$.
%On the one hand, we can relate the inputs and outputs through a simple linear-regression model 
%$\dataouti= \omega^*\datainE_i+\noiseE_i$ parameterized by $\omega^*\in\R$. 
%The least-squares estimate for~$\omega^*$ minimizes the objective function~$f_1\,:\,\omega\mapsto \omega^2+(1-\omega)^2$.
%The function $f_1$ is \Res{smooth and convex }(see the left panel of Figure~\ref{fig:ConVsNonCon}).
%
%On the other hand,
%we can also relate the inputs and outputs through a very simple linear neural-network model $\dataouti=\gamma^*\theta^*\datainE_i+\noiseE_i$ parametrized by $\gamma^*,\theta^*\in\R$.
%The least-squares estimate for $\gamma^*,\theta^*$ minimizes the objective function~$f_2\,:\,(\gamma,\theta)\mapsto(\gamma\theta)^2+(1-\gamma\theta)^2$.
%The earlier estimate and the one here are equivalent from a statistical perspective:
%we can simply identify~$\omega$ with the product~$\gamma\theta$.
%But the reparametrization changes the computational properties: 
%the function $f_2$ is not convex any more (see the right panel of Figure~\ref{fig:ConVsNonCon}). 

%Going from linear regression and other standard models to neural networks naturally leads to computational challenges;
%in particular, 
%the corresponding objective functions are usually non-convex,
%which means that
%optimization algorithms may easily get stuck in non-optimal stationary points.
%Thus,
%we argue that statistical guarantees in deep learning should concern stationary points rather than just global optima.
%Statistical theory of linear neural networks is of much interest in recent years; for example, \citet{dai2021representation} studies the representation costs of linear neural networks and \cite{saxe2013exact} show that deep linear networks exhibit nonlinear learning phenomena. 

%\begin{figure}[t]
%	\centering
%	\scalebox{1}{
	%		\includegraphics[width=6cm, height=5cm]{Figures/convex.pdf}}
%	\scalebox{1}{
	%		\includegraphics[width=6cm, height=5cm]{Figures/Nonconvex.pdf}}
%	\caption{Objective function of least-squares in linear regression (left panel) and in a neural-network model (right panel) for data  $(\datainE_1,\dataoutE_1)=(-1,0)$ and  $(\datainE_2,\dataoutE_2)=(1,1)$.
	%		The linear-regression function is convex while the neural-network function is highly non-convex.}
%	\label{fig:ConVsNonCon}
%\end{figure}
\paragraph{Paper contribution}
The three main technical contribution of this paper are as follows: 
\begin{enumerate}
	\item 
	We show that every (reasonable) stationary point of regularized  shallow linear neural networks and the points nearby  generalize essentially as well as the global optima (Theorem~\ref{OracleInSta} and Theorem~\ref{StaAppr}). 
	\item We extend our theories  to shallow ReLU neural networks for specific stationary points (Theorem~\ref{OracleInStaReLU}).%under assuming   the first layer weight matrix of the stationary point, as well as the target network be ``nearly identity'' 
	
	\item We determine the optimal rates for the tuning parameter across different networks and noise distributions (Theorem~\ref{OracleInStaHN}).
	%	 (Theorem~\ref{OracleInStaHN} of the Supplementary Material).
	%settings (network, noise distribution). 
\end{enumerate}

Of course, our theoretical framework is still far from the extremely complex pipelines of modern deep learning.
But our paper makes considerable progress in closing the gap between our theoretical understanding and practical experiences.
In particular, it (i)~strengthens the statistical foundations of deep learning and (ii)~gives a first mathematically rigorous proof of the empirical finding that  (ii.A)~approximate and (ii.B)~local optimization of neural networks is usually sufficient in practice.

\paragraph{Paper outline}
Section~\ref{Mainresult} states the statistical guarantees for the stationary points of the shallow linear neural network (Theorem~\ref{OracleInSta}) and the points nearby (Theorem~\ref{StaAppr}).
We extend our theories to shallow ReLU networks in Section~\ref{MainresultReLU} (Theorem~\ref{OracleInStaReLU}).
We support our theories with  numerical observations in Section~\ref{NumSec}. 
Section~\ref{RelatedWork} provides an overview of related works. 
%In Section~\ref{TechResult}, we study the behavior of the Hessian matrix of the population risk for shallow linear and ReLU networks (Proposition~\ref{PSDHessian} and Proposition~\ref{PSDHessianReLU}) and then employ tools from empirical-process theory to bound the absolute  difference between the gradient vector of the prediction and population risk (Lemma~\ref{EmpProcctwo}, Remark~\ref{RemarkReLU});
%these are the main ingredients for proving our Theorem~\ref{OracleInSta} and Theorem~\ref{OracleInStaReLU}.
We represent some of our technical results in Section~\ref{TechResult} and extend our theory for heavy-tailed noise in Sections~\ref{Hnoise}. 
We conclude our paper in Section~\ref{discussion}. 
More technical results, detailed proofs,  and  discussion on different assumptions are given in the Appendix.

\paragraph{Notations}
We use $\vectorize(\parameterout,\parameterin)$ to generate a vector of length $\R^{\nbrwidth+\nbrwidth\cdot\nbrinput}$ from a vector $\parameterout\in\R^{\nbrwidth}$ and a matrix $\parameterin\in\R^{\nbrwidth\times\nbrinput}$ (for generating the vector, we first push the elements of $\parameterout$ and then elements of $\parameterin$ row by row).  
We collect first-order partial derivatives (and subdifferentials for ReLU networks) of prediction risk $\objectiveF{\parameterout,\parameterin}$ and population risk  $\objectiveFP{\parameterout,\parameterin}$ with respect to the $\ParamV\deq\vectorize(\parameterout,\parameterin)$ in the gradient vectors $\DervSam\in\R^{\nbrwidth+\nbrwidth\cdot\nbrinput}$ and $\DervPop\in\R^{\nbrwidth+\nbrwidth\cdot\nbrinput}$, respectively.
We use the notation $\norm{\cdot}$ for a general vector norm and $\normM{\cdot}$ for a  general matrix norm. 
We also define $\normone{\parameterout}\deq\sum_{\jn=1}^{\nbrwidth}|\parameteroutE_{\jn}|$ and $\normoneM{\parameterin}\deq\sum_{\jn=1}^{\nbrwidth}\sum_{\kn=1}^{\nbrinput}|\parameterinjk|$.
To reduce the amount of notations, we use some notation slightly differently depending on whether we treat linear or ReLU networks. 





\section{Statistical guarantees for shallow linear neural networks}\label{Mainresult}

Consider inputs $\datain_1,\dots,\datain_{\nbrsamples}\in\R^{\nbrinput}$ and corresponding outputs $\dataoutE_1,\dots,\dataoutE_{\nbrsamples}\in\R$ that are connected via
\begin{linenomath}
	\begin{equation}\label{target}
		\dataouti~=~\TrueFuni+\noisei
	\end{equation}
\end{linenomath}
for an unknown target function $\TrueFun\,:\,\R^{\nbrinput}\to\R$ and unknown stochastic noise $\noiseN_1,\dots,\noiseN_{\nbrsamples}\in\R$.
Deep learning is about using the available data to approximate the unknown target function~$\TrueFun$ by a neural network.
We first focus on linear neural networks,
a well-accepted toy model for more general deep learning pipelines~\citep{saxe2013exact};
hence, we consider 
\begin{linenomath}
	\begin{equation*}
		\datain~\mapsto~\parameterout\tp\parameterin\datain\,,
	\end{equation*}
\end{linenomath}
where 
\begin{linenomath}
	\begin{equation*}
		(\parameterout,\parameterin)~\in~\ParamSpaceM\,\deq\,\bigl\{(\parameterout,\parameterin)~\in~\R^{\nbrwidth}\times\R^{\nbrwidth\times\nbrinput}\bigr\}\,.
	\end{equation*}
\end{linenomath}
We extend this setup to ReLU activation in the following section.





To avoid unnecessary digression here, we impose three mild assumptions. 
The assumptions are by no means necessary and relaxed in the following sections.
\begin{assumption}[Model Assumptions]\label{assump}
	We assume that:
	\begin{enumerate}
		\item  The target function can be approximated by such a neural network in the first place:
		there is a pair $ (\parameteroutS,\parameterinS)\in\ParamSpaceM$
		such that   $\normone{\parameteroutS},\normoneM{\parameterinS}\leq \sqrt{\log{\nbrsamples}}$ 
		and $\TrueFun[\datain]=\parameteroutS\tp \parameterinS \datain$ for all $\datain\in\R^{\nbrinput}$.
		\item The $\dataini$'s are independent and centered sub-Gaussian random vectors with independent coordinates.
		\item The $\noiseE_i$'s are independent centered Gaussian random variables with standard deviation $\sigma$ and are independent of $\dataini$'s.
	\end{enumerate}
\end{assumption}
The first part of Assumption~\ref{assump} ensures a sharp focus on  statistical guarantees rather than the approximation properties of neural networks, we assume that
the target function is itself a neural network with reasonably small parameters.
%\footnote{The bound $\sqrt{\log{\nbrsamples}}$ here and on the next page is merely for convenience: 
	%it can be replaced by any fixed constant or another function that is increasing mildly in the sample size~$\nbrsamples$.}
%(see also Appendix Section~\ref{Cost-norm} and Theorem~\ref{OracleInStaq} for a detailed description of this assumption; 
%\textcolor{\draftcolort}{our Theorem~\ref{OracleInStaq} provides a generalized version of our Theorem~\ref{OracleInSta} by relaxing the first part of  Assumption~\ref{assump}.})
%Note that parametrization  of neural networks is ambiguous:
%there are provably infinitely many pairs $ (\parameteroutS,\parameterinS)\in\ParamSpaceM$ that satisfy those conditions---compare to~\citet[Proposition~1]{taheri2021};
A detailed description of the assumption is provided in Section~\ref{Cost-norm} of the Appendix; the assumption is relaxed in  Theorem~\ref{OracleInStaq}.
Note that the parametrization  of neural networks is ambiguous:
there are infinitely many pairs $ (\parameteroutS,\parameterinS)\in\ParamSpaceM$ that satisfy those conditions---compare to~\citet[Proposition~1]{taheri2021};
for further reference,
we define $\ParamVS\deq\vectorize(\parameteroutS,\parameterinS)$ for a fixed but arbitrary such pair of parameters.
%\textcolor{red}{please describe why the second part of the assumption is harmless, too!}
The second part of the assumption  on the input simplifies our theoretical analysis. 
%Although this assumption is not necessarily true in practice,  that is a common assumption in the literature and
%can be extended more generally in future works. 
Although it may not always strictly hold in practice, it is widely adopted in the literature as a convenient modeling device; see, for example~\cite{Vershynin2018,wainwright2019high,Sara2000}. Intuitively, each coordinate of $\datain$ can be interpreted as a feature extracted from the raw data, and independence is then a simplifying assumption. Moreover, the mean-zero sub-Gaussian property is often assumed to capture concentration behavior of feature vectors in high-dimensional models and can be achieved through data preprocessing.
The third part of the assumption, once more, simplifies the presentation here;
extensions to other types of noise,
including sub-Gaussian and sub-exponential noise are provided in Section~\ref{Hnoise}.

%	We focus on linear neural networks,
%	which are simple enough to be analyzed theoretically and yet display the relevant properties of any network.
%	We then extend our results to ReLU activation function in Section~\ref{MainresultReLU}.




We assume our regression setup ($\dataouti\in\R$) rather than a classification setup ($\dataouti\in\{0,1\}$ or $\dataouti\in\{1,\dots,k\}$) because the unbounded outputs make regression considerably more challenging to analyze mathematically.
In other words, our regression results transfer readily to classification.
The usual loss function in regression is least squares.
In deep-learning practice, however, least squares (and similarly logistic loss in classification) is complemented with dropout~\citep{srivastava2014dropout,Salehinejad2019},
batch normalization~\citep{ioffe2015batch},
low-rank approximation~\citep{Denil2013},
and so forth,
which yield implicit regularization,
or least squares is even complemented with explicit regularization directly~\citep{Alvarez16,lemhadri2021lassonet,HEBIRI2025106195}.
It is well understood that implicit regularization is related to explicit regularization~\citep{lutke2024dropout}.
Thus, to mimic deep-learning practice,
we consider least-squares complemented by (elementwise) $\ell_1$-regularization:
\begin{linenomath}
	\begin{equation}\label{ls}
		(\estimatorout,\estimatorin)~\in~\argmin_{(\parameterout,\parameterin)\in\ParamSpaceM}\biggl\{\frac{1}{\nbrsamples}\sum_{i=1}^{\nbrsamples}\bigl(\dataouti-\parameterout\tp\parameterin\dataini\bigr)^2+\tuning\normone{\vectorize(\parameterout,\parameterin)}\biggr\}\,,
	\end{equation}
\end{linenomath}
where $\tuning\in[0,\infty)$ is a tuning parameter to be calibrated (see~\cite{sardy2020needles} for some theory insights).
Such estimators 
are standard in machine learning and statistics~\citep{Lederer2021HD,eldar2012compressed}.
\textcolor{\draftcolort}{Despite $\ell_1$-norm  is non-smooth, it often poses very little problems in terms of computations (see~\cite{friedman2010regularization}). Also recently, the $\ell_1$-norm has been effectively used to promote sparsity in neural networks~\citep{lemhadri2021lassonet}.}


As usual, we measure the  (in-sample-)prediction risk by 
\begin{linenomath}
	\begin{equation*}
		\objectiveF{\parameterout,\parameterin}~\deq~ \frac{1}{\nbrsamples}\sum_{i=1}^{\nbrsamples}\bigl(\dataouti-\parameterout\tp\parameterin\dataini\bigr)^2
	\end{equation*}
\end{linenomath}
with $\datainM\deq(\datain_1,\dots,\datain_{\nbrsamples})\tp\in\R^{\nbrsamples\times\nbrinput}$ and the generalization risk by
\begin{linenomath}
	\begin{equation*}
		\objectiveP[\parameterout,\parameterin]~\deq~\E_{(\datain,\dataoutE)}\Bigl[\bigl(\dataoutE-\parameterout\tp\parameterin\datain\bigr)^2\Bigr]
	\end{equation*}
\end{linenomath}
with the expectation over a new sample $(\datain,\dataoutE)$ (that has the same distribution as $\datain_1,\dots,\datain_{\nbrsamples}$ and $\dataoutE_1,\dots,\dataoutE_{\nbrsamples}$).
We call $\ParamSta\deq\vectorize(\StaOut,\StaIn)$  a \emph{stationary point} of the objective in~\eqref{ls} if it satisfies~\citep[Page~194]{bertsekas1997nonlinear};\citep[Equation~6]{elsener2018sharp};\citep[Equation~5]{loh2015}
%\citep[Page~194]{bertsekas1997nonlinear}
\begin{equation}\label{StaP}
	\bigl(\DervSamSta\bigr)\tp(\ParamV-\ParamSta)+\tuning\tildez\tp(\ParamV-\ParamSta)~\ge~ 0~~~~~\forall~ \ParamV=\vectorize(\parameterout,\parameterin)~~ \text{with}~~(\parameterout,\parameterin)\in~\ParamSpaceM
\end{equation}
for appropriate $\tildez\in\boldsymbol{\partial}\normone{\ParamSta}$ (where $\boldsymbol{\partial}\normone{\ParamSta}$ is the subdifferential of the regularizer at $\ParamSta$). 
For an interior point $\ParamSta$, our definition of stationary points in~\eqref{StaP} reduces to the usual zero-subgradient condition.
%for  $(\ParamV-\ParamSta)\eqd\Delta\ParamV$,  it implies $ (\DervSamSta)\tp \Delta\ParamV+\tuning\tildez\tp \Delta\ParamV~\ge~  \boldsymbol{0}$ and $ (\DervSamSta)\tp \Delta\ParamV+\tuning\tildez\tp \Delta\ParamV~\le~  \boldsymbol{0}$, that reduces to $ (\DervSamSta)\tp \Delta\ParamV+\tuning\tildez\tp \Delta\ParamV= \boldsymbol{0}$.

We call a stationary point $
\ParamSta$ \emph{reasonable} once $\normone{\StaOut},\normoneM{\StaIn}\leq \sqrt{\log{\nbrsamples}}$---again to avoid unnecessary complication (we refer to  the Appendix Section~\ref{Sec-ResAs} for a detailed description of the reasonability assumption).
Due to the ambiguity of neural networks, there are  infinitely many equivalent stationary and reasonable stationary points;
importantly, our guarantees hold for every (reasonable) stationary point and target~$\ParamVS$.



We say that a network indexed by $(\StaOut,\StaIn)$ generalizes well if
\begin{linenomath}
	\begin{equation*}
		\objectiveP[\StaOut,\StaIn]~\approx\,\operatorname{risk}[\parameteroutS,\parameterinS]\,,
	\end{equation*}
\end{linenomath}
that is, the network generalizes essentially as well as the best network.
In the following, we show that not only the ``statistical'' network indexed by $(\estimatorout,\estimatorin)$ but also every ``practical'' network indexed by a reasonable stationary point $(\StaOut,\StaIn)$ of the objective function in~\eqref{ls} generalizes well.

Moreover, 
we call the total number of parameters in the network $\EfDim\deq\nbrwidth+\nbrwidth\cdot\nbrinput$ the problem's effective dimension and
\begin{linenomath}
	\begin{equation}\label{oracletuning}
		\tuningopt~\deq~\DisP(\log{\nbrsamples})^{3/2}\sqrt{\frac{\log(\nbrsamples\EfDim)}{\nbrsamples}}
	\end{equation}
\end{linenomath}
the oracle tuning parameter, where $\DisP\in(0,\infty)$ is a constant that depends only on 
the distributions of the inputs and noise.
It has been shown that $\tuningopt$ is indeed an optimal tuning parameter of~\eqref{ls} in some sense~\citep{taheri2021}.




We then get the following result for a new sample pair $(\datain,\dataoutE)$ with the same distribution as $\datain_1,\dots,\datain_{\nbrsamples}$ and $\dataoutE_1,\dots,\dataoutE_{\nbrsamples}$.

\begin{theorem}[Statistical Guarantees for Reasonable Stationary Points of Shallow Linear Networks]\label{OracleInSta}
	Under the Assumption~\ref{assump}  
	any  reasonable stationary point $(\StaOut,\StaIn)$ 
	of the objective function in~\eqref{ls} with $\tuning\ge \tuningopt$ satisfies the risk bound
	\begin{linenomath}
		\begin{equation}\label{main_ineq}
			\objectiveP[\StaOut,\StaIn]~\leq~\objectiveP[\parameteroutS,\parameterinS]+5\tuning\sqrt{\log\nbrsamples}
		\end{equation}
	\end{linenomath}
	with probability at least    
	$1-1/2\nbrsamples$. 
	If $\tuning=\tuningopt$,
	the bound becomes
	\begin{linenomath}
		\begin{equation}\label{Main_rates}
			\objectiveP[\StaOut,\StaIn]~\leq~\objectiveP[\parameteroutS,\parameterinS]+\DisP(\log{\nbrsamples})^{2}\sqrt{\frac{\log(\nbrsamples\EfDim)}{\nbrsamples}}\,.
		\end{equation}
	\end{linenomath}
	% \begin{equation*}
		%  \objectiveP[\StaOut,\StaIn]~\leq~\objectiveP[\parameteroutS,\parameterinS]+4\DisP(\log{\nbrsamples})^{2}\sqrt{\frac{\log(\nbrsamples\nbrinput\EfDim)}{\nbrsamples}}+\DisP(\log{\nbrsamples})^{3/2}\sqrt{\frac{\log(\nbrsamples\nbrinput\EfDim)}{4\nbrsamples^3}}\Bigl(4\log{\nbrsamples}+\frac{1}{2\nbrsamples}\Bigr)
		% with probability at least   
		% $1-8\lceil\log{(4\nbrsamples} )\rceil/{\nbrsamples}$.
		% (over the input and output data $\datain_1,\dots,\datain_{\nbrsamples},\dataoutE_1,\dots,\dataoutE_{\nbrsamples}$).
	\end{theorem}
	%A high-level  proof for Theorem~\ref{OracleInSta} is provided in Section~\ref{App}, while the  detailed  version is deferred to  the Supplementary. 
	
	% \begin{corollary}\label{BestApprox}
		% Assume that the conditions of Theorem~\ref{OracleInSta} are satisfied and that $\tuning=\tuningopt$.  Then, we have
		% \begin{equation*}
			%  \objectiveP[\StaOut,\StaIn]~\leq~\objectiveP[\parameteroutS,\parameterinS]+\frac{640}{\sqrt{\DisC\nbrsamples}}\DisP(\log{\nbrsamples})^{2}\sqrt{{\log(\nbrsamples\nbrinput\EfDim)}}+\frac{80}{\sqrt{\DisC\nbrsamples^3}}\DisP(\log{\nbrsamples})^{3/2}\sqrt{{\log(\nbrsamples\nbrinput\EfDim)}}
			% \end{equation*}
		% with probability at least   
		% $1-8\lceil\log{(4\nbrsamples} )\rceil/{\nbrsamples}$.
		
		% \end{corollary}
	
	Theorem~\ref{OracleInSta} proves the fact that for properly chosen tuning parameter~$\tuning$ and large enough sample sizes,
	any reasonable stationary point of~\eqref{ls} generalizes essentially as well as $\ParamVS$.
	Our results essentially have the same rates as the ones in the literature~\citep[Theorem~3]{taheri2021};\citep[Proposition~3]{2021LedererSparse}, 
	who prove that the prediction risk is at most of order $O((L/2)^{1/2-L}\log(p)\allowbreak\log(n)/\sqrt{n})$) for $\ell_1$-regularized neural networks with depth $L$ and $p$ parameters.
	However, in stark contrast to previous results, our theories apply to all reasonable stationary points (including saddle points) rather than to the global optimum of the objective function only. 
	%While works such as~\citet{kawaguchi2016deep} argue about the absence  of local min in linear networks under some assumptions,  saddle points remain problematic. 
	Although works like~\citet{kawaguchi2016deep} and \cite{zhou2018critical} argue about the absence  of local minima in linear networks,  saddle points still exist in linear neural networks (see~\citet[Theorem~2]{zhou2018critical}). 
	Furthermore, saddle points continue to pose challenges:
	\citet{lee2019first} demonstrate that gradient-based algorithms can escape strict saddle points, but
	non-strict saddle points are problematic and also exist in linear neural networks in general~\citep[Paragraph following their Theorem~2]{zhou2018critical}.
	We refer to our illustrative Example~\ref{exm:relu} (in the Appendix) to clearly illustrate the presence of sub-optimal critical points in our considered setup. 
	Also, a recent study by~\cite{achour2024loss}  demonstrates that  for shallow linear neural networks with least squares loss,  all saddle points are strict under some assumptions (see \citet[Assumption~1]{achour2024loss}. 
	
	
	To emphasize the significance of using regularized objectives, it's worth mentioning that the rate of ordinary least-squares in linear regression is $O(d/n)$, where $d$ gives the number of parameters and $n$  the number of data examples~\citep[Equation~1.5]{Lederer2021HD}.
	But for high-dimensional settings with $d \gg n$, least-squares are prone to overfitting, so regularization can be employed for improvement. 
	For example,  lasso with sufficiently large tuning parameter (in linear regression) gives predictions bounds at most bounded by $\sqrt{\log(d)/n}$~\citep[Page~174]{Lederer2021HD}. 
	Also, a different prediction bound for lasso called ``power-two bound"  is presented in~\citet[Page~188]{Lederer2021HD} that holds under strong conditions but it is far from the context of this paper. 
	Overfitting is even more problematic for complex models like neural networks with a huge number of parameters $p$.
	The focus has just shifted to networks involving sparsity to improve  prediction bounds from $p/n$  to $\sqrt{\log(p)/n}$, which  also appears in our results (see~\eqref{Main_rates} for example).
	
	%\Res{Also,  most of the theory and applied deep learning papers  focus on classification setting, 
		%while the regression setting is much more challenging.
		%Unbounded loss  makes regular techniques like McDiarmid's inequality~\citep[Lemma~3.3]{mcdiarmid1989method} not applicable for regression settings. 
		%So, our empirical processes approach seems more general and can also be applied to classification. 
		%}
	
	Note that in finite time,  stationary points can be computed just approximately using gradient-based algorithms. 
	Now, we  extend our results in Theorem~\ref{OracleInSta} to the points that are close but not necessarily equal to a stationary points.
	We define a pair $(\StaOutAp,\StaInAp)$ as a $\AppSta-$approximate stationary point if it satisfies
	\begin{linenomath}
		\begin{equation}\label{approx-sta}
			\bigl|\objectiveF{\StaOutAp,\StaInAp}+\tuning\normone{\ParamStaAp}-\objectiveF{\StaOut,\StaIn}-\tuning\normone{\ParamSta}\bigr|~\le~\AppSta
		\end{equation}
	\end{linenomath}
	for a $\AppSta\in[0,\infty)$.
	Our definition of approximate stationary points in~\eqref{approx-sta} is closely related to the typical definitions in the literature that impose some bounds on the norm of the gradient vectors (see  Appendix Section~\ref{Sec:DynApS}  for a detailed description).
	Employing gradient-based algorithms (in finite time), we can expect to get close to a stationary point in the sense that  $\ParamStaAp\approx\ParamSta$~\citep{ghadimi2013stochastic,lei2019stochastic}. 
	Then also $\normone{\ParamStaAp}\approx\normone{\ParamSta}$, which means that
	an approximation of a reasonable stationary point is also reasonable once $\AppSta$ is small enough.
	Then, we extract statistical guarantees  for every practical network indexed by an approximate-reasonable stationary   as follows:
	\begin{theorem}[Statistical Guarantees for  Approximate Stationary Points of Shallow Linear Networks]\label{StaAppr}
		Suppose that $(\StaOutAp,\StaInAp)$ is a $\AppSta-$approximate stationary point and that the conditions of Theorem~\ref{OracleInSta} are satisfied.
		Then, we have
		\begin{linenomath}
			\begin{equation}\label{main_ineq_app}
				\objectiveFP{\StaOutAp,\StaInAp}~\le~\objectiveP[\parameteroutS,\parameterinS]+8\tuning\sqrt{\log\nbrsamples}+\AppSta
			\end{equation}
		\end{linenomath}
		with probability at least $1-1/\nbrsamples$.
		If $\tuning=\tuningopt$,
		the bound becomes
		\begin{linenomath}
			\begin{equation}
				\objectiveP[\StaOutAp,\StaInAp]~\leq~\objectiveP[\parameteroutS,\parameterinS]+\DisP(\log{\nbrsamples})^{2}\sqrt{\frac{\log(\nbrsamples\EfDim)}{\nbrsamples}}+\AppSta\,.
			\end{equation}
		\end{linenomath}
	\end{theorem}
	%The proof of Theorem~\ref{StaAppr} is given in the  Supplementary material~\ref{proofs}.
	
	
	The bounds match the earlier ones with only two small differences: 1.~a summand $\AppSta$ is added to our statistical bounds and 2.~the factor 5 in~\eqref{main_ineq} is replaced by a factor of 8 in~\eqref{main_ineq_app}.
	Let's note that gradient-based algorithms with sufficiently many steps $O(\nbrsamples^2)$ ensure that $\AppSta\ll 1/\sqrt{\nbrsamples}$~\citep[Theorem~2.1]{ghadimi2013stochastic}. 
	We refer to our  Appendix Section~\ref{DynamicAppSta} for more details regarding the dynamical accessibility of approximate stationary points. 
	Theorem~\ref{StaAppr} might look like a simple extension of Theorem~\ref{OracleInSta},
	but the fact that~\eqref{approx-sta} involves the (in-sample-)prediction risk and the   sparsity factors makes the proof considerably more involved.
	
	\section{Statistical guarantees for shallow ReLU neural networks}\label{MainresultReLU}
	This section generalizes our theories in Section~\ref{Mainresult} to shallow ReLU neural networks of the form 
	\begin{linenomath}
		\begin{equation*}
			\datain~\mapsto~\parameterout\tp\relu(\parameterin\datain)\,,
		\end{equation*}
	\end{linenomath}
	for $(\parameterout,\parameterin)~\in~\ParamSpaceM\,=\,\{(\parameterout,\parameterin)~\in~\R^{\nbrwidth}\times\R^{\nbrwidth\times\nbrinput}\}$.
	The activation function 
	$\relu(\cdot)$ corresponds to the well-known ReLU defined as  $\relu(\boldsymbol{z})\deq (\max(0,z_1),\dots,\max(0,z_{\nbrwidth})) $ for $\boldsymbol{z}\in \R^{\nbrwidth}$, which 
	its efficacy has been extensively studied~\citep{pan2016expressiveness,raghu2017expressive}.
	We then approximate the unknown target function~$\TrueFun$ in~\eqref{target} employing shallow ReLU neural networks.
	For simplifying the proofs, we assume in this section  that  $\nbrinput=\nbrwidth$ that implies  matrix $\parameterin$ to be  squared.
	%We employ exactly same notations used for linear networks in Section~\ref{Mainresult} as well (for simplicity), despite networks in this section are considered as shallow-ReLU networks (as defined above). 
	We then consider least-squares complemented by  $\ell_1$-regularization  for shallow ReLU neural networks:
	\begin{linenomath}
		\begin{equation}\label{lsReLU}
			(\estimatorout,\estimatorin)~\in~\argmin_{(\parameterout,\parameterin)\in\ParamSpaceM}\biggl\{\frac{1}{\nbrsamples}\sum_{i=1}^{\nbrsamples}\bigl(\dataouti-\parameterout\tp\relu(\parameterin\dataini)\bigr)^2+\tuning\normone{\vectorize(\parameterout,\parameterin)}\biggr\}\,.
		\end{equation}
	\end{linenomath}
	
	\begin{assumption}[Model Assumptions (ReLU)]\label{assumpReLU}
		%		We assume that the target function can be approximated by such a neural network, that is, 
		%		there is a pair $ (\parameteroutS,\parameterinS)\in\ParamSpaceM$
		%		such that   $\normone{\parameteroutS},\normoneM{\parameterinS}\leq \sqrt{\log{\nbrsamples}}$ and  $\parameterinS\approx \boldsymbol{I}_{\nbrwidth}$ \textcolor{\draftcolort}{(that is $\parameterinS= \boldsymbol{I}_{\nbrwidth}+A$ for $A\in \R^{\nbrwidth\times \nbrwidth}$ , in which, $\normM{A}\approx 0$)},
		%		and that $\TrueFun[\datain]=\parameteroutS\tp \relu(\parameterinS \datain)$ for all $\datain\in\R^{\nbrinput}$.		
		We assume that the target function can be approximated by such a neural network, that is, 
		there is a pair $ (\parameteroutS,\parameterinS)\in\ParamSpaceM$
		such that   $\normone{\parameteroutS},\normoneM{\parameterinS}\leq \sqrt{\log{\nbrsamples}}$ 
		and  active rows in $\parameterinS$ are approximately perpendicular to each other
		% has approximately orthogonal rows ($\parameterinS \parameterinS\tp =\boldsymbol{I}_{\nbrwidth}+A$ for $A\in \R^{\nbrwidth\times \nbrwidth}$  in which, $\normM{A}\approx 0$)  %small  cross alignment ($\parameterinS$),
		%and   $\parameterinS= \boldsymbol{I}_{w}+A$ for $A\in \R^{w\times w}$, in which, $\normM{A} \le \tau$ with $\tau\to 0$,
		and that $\TrueFun[\datain]=\parameteroutS\tp \relu(\parameterinS \datain)$ for all $\datain\in \R^{\nbrinput}$.		
	\end{assumption}
	\noindent
	The term active rows in a matrix $\Theta$ are approximately perpendicular to each other in our assumption above means, for any two distinct active rows $\Theta_{j,\cdot}$ and $\Theta_{j',\cdot}$ (where $\Theta_{j,\cdot},\Theta_{j',\cdot} \neq \mathbf{0}$), their inner product is negligible, that is $\langle \Theta_{j,\cdot}, \Theta_{j',\cdot} \rangle \approx 0.0$. 
	Assumption~\ref{assumpReLU} 
	%	 keeps our proofs tractable.
	%	It 
	stipulates that the target function is itself a shallow ReLU neural network with reasonably small parameters
	and that the active rows of the first layer are approximately orthogonal.
	%	is not too far from isotropic $\parameterinS\approx \boldsymbol{I}_{\nbrwidth}$ (recall that $\nbrwidth=\nbrinput$ in this section).
	%	For simplicity, we use the notation $\Theta\approx \boldsymbol{I}_{\nbrwidth}$ for a square matrix $\Theta~\in \R^{\nbrwidth\times \nbrwidth}$, when the off-diagonal elements of that matrix are close to zero and the diagonal elements are close to one.
	%	Formulated differently, we say $\Theta\approx \boldsymbol{I}_{\nbrwidth}$, if $\Theta$ can be represented as  a sum over a square matrix $A \in \R^{\nbrwidth\times \nbrwidth}$ and identity matrix $\boldsymbol{I}_{\nbrwidth}$, that is, $\Theta= \boldsymbol{I}_{\nbrwidth}+A$, in which,  square matrix $A$ has a small spectral norm. 
	Versions of these assumptions are very common in the literature~\citep{hardt2016identity,bartlett2018gradient}; we discuss this assumption further in the paragraph following Theorem~\ref{OracleInStaReLU}.
	We then define the (in-sample-)prediction  and generalization risk  for shallow ReLU neural networks as (we employ the same notation as used in the linear case) 
	\begin{equation*}
		\objectiveF{\parameterout,\parameterin}~\deq~ \frac{1}{\nbrsamples}\sum_{i=1}^{\nbrsamples}\bigl(\dataouti-\parameterout\tp\relu(\parameterin\datain)\bigr)^2
	\end{equation*}
	and
	\begin{equation*}
		\objectiveP[\parameterout,\parameterin]~\deq~\E_{(\datain,\dataoutE)}\Bigl[\bigl(\dataoutE-\parameterout\tp\relu(\parameterin\datain)\bigr)^2\Bigr]\,.
	\end{equation*}
	We then get the following result for a new sample pair $(\datain,\dataoutE)$ with the same distribution as $\datain_1,\dots,\datain_{\nbrsamples}$ and $\dataoutE_1,\dots,\dataoutE_{\nbrsamples}$.
	
	
	\begin{theorem}[Statistical Guarantees for Reasonable Stationary Points of Shallow ReLU Networks]\label{OracleInStaReLU}
		Under the second and third parts of  Assumption~\ref{assump}  and  Assumption~\ref{assumpReLU},
		any  reasonable stationary point $(\StaOut,\StaIn)$ of the objective function in~\eqref{lsReLU} where active rows of  $\StaIn$   are approximately perpendicular to each other and  that  off-diagonal elements of  $\StaIn\parameterinS\tp$ and $\parameterinS\StaIn\tp$ are    approximately zero ($|(\StaIn\parameterinS\tp)_{jj'}|\approx |(\parameterinS\StaIn\tp)_{jj'}|\approx 0.0$ for $j\ne j'$)
		%		with $\StaIn\approx \boldsymbol{I}_{\nbrwidth}$ \textcolor{\draftcolort}{(that is $\StaIn= \boldsymbol{I}_{\nbrwidth}+A'$ for $A'\in \R^{\nbrwidth\times \nbrwidth}$ , in which, $\normM{A'}\approx 0$)}
		%with $\StaIn= \boldsymbol{I}_{w}+A'$ for $A'\in \R^{w\times w}$, in which, $\normM{A'}\le \tau$ with $\tau\to 0$ 
		with $\tuning\ge \tuningopt$ satisfies the risk bound
		\begin{linenomath}
			\begin{equation}
				\objectiveP[\StaOut,\StaIn]~\leq~\objectiveP[\parameteroutS,\parameterinS]+5\tuning\sqrt{\log\nbrsamples}
			\end{equation}
		\end{linenomath}
		with probability at least    
		$1-1/2\nbrsamples$. 
		%	If $\tuning=\tuningopt$,
		%	the bound becomes
		%	\begin{linenomath}
			%		\begin{equation}
				%			\objectiveP[\StaOut,\StaIn]~\leq~\objectiveP[\parameteroutS,\parameterinS]+\DisP(\log{\nbrsamples})^{2}\sqrt{\frac{\log(\nbrsamples\EfDim)}{\nbrsamples}}\,.
				%		\end{equation}
			%	\end{linenomath}
	\end{theorem}
	Note that  Theorem~\ref{OracleInStaReLU} is an extension of our Theorem~\ref{OracleInSta} for shallow ReLU neural networks under the assumption that the active rows of the first layer weight matrix (for stationary point and the target) being approximately orthogonal (one simple example is near-identity matrices). 
		Orthogonal weight matrices  is needed mainly for studying Hessian behavior for shallow ReLU network's (proof of Proposition~\ref{PSDHessianReLU}, Step~2). Employing this assumption, we can prove that for cases with small correlation between rows and with Gaussian input, we can find a closed-form solution (approximately) for $\E_{\boldsymbol{x}}[\relu(\Theta \boldsymbol{x})_j \relu(\Theta \boldsymbol{x})_{j'}] $.
	Our Assumption~\ref{assumpReLU} is weaker than it seems as previous works have studied variants of this assumption for neural networks from different perspectives:  for example,~\citet{hardt2016identity} shows that certain networks have a global minimum close to the identity parameterization. They study the expressiveness of Residual Networks under the assumption that enough neurons are available~\citep[Theorem~3.2]{hardt2016identity}. Interesting is that, since our rates grow just in $\log p$ , our framework is perfectly fit for such wide networks. 
	Additionally, \cite{bartlett2018representing} explore the representation of smooth functions as compositions of near-identity functions, highlighting implications for deep network optimization.
	\citet{bartlett2018gradient}  prove the rate of convergence of gradient-based optimization under identity initialization for deep linear networks.
	\citet{li2017convergence}   analyze the convergence  of stochastic gradient descent  for shallow ReLU networks, with nearly identity initialization; they state that ``(ReLU) networks with small average spectral norm already have good performance.''
	\textcolor{\draftcolort}{Altogether, we believe that our  assumption makes sense not only from an expressivity standpoint~\citep[Theorem~3.2]{hardt2016identity} but also regarding the optimization landscape~\citep{li2017convergence}. Yet, of course, it would be interesting to study the subtleties even further.}
	%	Although these works have  a different perspective than ours, their results are  still 
	%	relevant, as they explore the significance of identity initialization in deep learning. 
	While studies demonstrate the existence of local minima and saddle points in ReLU networks~\citep{fukumizu2000local,safran2018spurious,yun2018small}, we argue that some of those suboptimals  still yield satisfactory results. 
	Essentially, Theorem~\ref{OracleInStaReLU} suggests that for a sufficiently large tuning parameter, the optimization explores locally well-curved network spaces in the vicinity of specific stationary points, such that any stationary point  generalizes as effectively as a global minimum.
	\textcolor{\draftcolort}{In fact, our work concerns local curvature around the ground truth in neural networks, which we believe is valuable given the infinite number of such ground truths in neural networks, while globally favorable curvature is far from practical reality in deep learning.}
	We employ our result in Proposition~\ref{PSDHessianReLU} and  Remark~\ref{RemarkReLU} proving our Theorem~\ref{OracleInStaReLU}. 
Also, an extension of Theorem~\ref{StaAppr} to shallow ReLU networks can be obtained by combining Theorem~\ref{OracleInStaReLU} with additional machinery from empirical process theory, following the same line of reasoning as in the proof of Theorem~\ref{StaAppr}.
	However, we omit this extension here to avoid redundancy.
	Also, we conjecture that our main theories can be extended to deep neural networks (see our simulations in Section~\ref{moreExperiments}), provided that suitable local curvature properties of the corresponding networks can be established. This presents an intriguing direction for future research.
	
	\paragraph{Further discussion of our Assumption~\ref{assumpReLU}}
	Our results suggest that low correlation between the rows of the first-layer weight matrix 
	$\widetilde\Theta$  is desirable, as it leads to a well-conditioned Hessian and better generalization. This observation is closely related to the benefits of random initialization: for large 
	$d$, random Gaussian weights yield nearly orthogonal rows with high probability (see \citet[Remark~3.2.5]{Vershynin2018}). However, orthogonality is not only needed at initialization but also for the estimator $\widetilde{\Theta}$ after training, which motivates arguments ensuring that training preserves this structure. Related studies show that fixing the first layer at its random initialization while only training the last layer can still achieve good generalization~\citep{rosenfeld2019intriguing}, suggesting that there exist network configurations where the first-layer rows form an approximately orthogonal system, leading to favorable error bounds. Finally, while some of the literature attributes low-rank structure in shallow networks to strong correlations among rows~\citep{kou2023implicit}, in our norm-one regularized setting low rank instead arises through sparsity: many rows might become inactive, while the surviving rows remain diverse and nearly orthogonal, which is enough for our results to hold.
	One can also considers group lasso to offer an alternative means of promoting structured sparsity.
	This alternative path to low-rank structure avoids redundancy, preserves conditioning, and further explains why such solutions generalize well.

	\section{Numerical observations}\label{NumSec}	
	We provide here some numerical observations to clarify  theories  of Section~\ref{Mainresult} and Section~\ref{MainresultReLU}. 
	We minimize a  least-squares complemented by $\ell_1$-regularization for shallow neural networks with linear and ReLU activation functions. 
	We set our tuning parameter on the order of $\log(np)/\sqrt{n}$ based on our experiments.
	We consider 
	neural networks with $\nbrinput=\nbrwidth=10$, that are trained over  500  and tested over 300 data sample generated from a  standard normal distribution and labeled by a sparse-target network (having the same structure as the considered model) plus a Gaussian noise.
	Note that here, we train the networks in a finite time, that means,  trained networks are just  an approximation of a stationary point (due to the non-convexity). 
	We report the relative training error and the relative test error for a potential global optimum, an approximate stationary point, and a randomly generated network (a network with randomly assigned weights)
	for linear and ReLU networks in Table~\ref{Tab-optim}, that is, the training (test) error of the ``approximate stationary point'' divided by the training (test) error of the ``potential global optimum'' (for the corresponding network).
	Potential global optimum and approximate stationary point (for each setting,  linear or ReLU) are reached over multiple times of training on a fixed data set and assigned by the  trained networks with the lowest and  highest training error, respectively.
	\textcolor{\draftcolort}{More precisely, we do the optimization (solving~\eqref{ls} and~\eqref{lsReLU}) from multiple, diverse initial points ($1000$ times). 
			We use PyTorch’s default initialization, where weights are drawn from a uniform distribution in $[-1/\sqrt{\EfDim}, 1/\sqrt{\EfDim}]$, with $\EfDim$ denoting the number of input features to the layer (see our results with different initialization methods in our  Section~\ref{moreExperiments}).
			This helps explore different regions of the search space and increases the chances of finding different local and global optimum. Note that there are infinitely many critical points for neural networks in view of the network's rescaling properties.
		We use stochastic gradient descent with a small convergence threshold to ensure that the optimization process does not stop early.
		We analyze the distribution of the reached training errors (over the  $1000$ different optimization runs with random initialization). For this, we divide the training errors into two clusters via k-means. Then, we do a t-test over the training errors in the two classes. The t-test reveals a statistically significant difference between the training errors in two groups ($p_{\operatorname{value}}<0.0001$), which supports the claim that the ``potential global optimum'' and ``approximate stationary points'' differ, that is, the approximate stationary points are not just other global optima.
		We then report the parameters that lead to the lowest training error as a ``potential global optimum'' and the parameters that lead to the highest training error as ``approximate stationary point''.}
	We reference to Figure~\ref{fig:Optim_Linear&Relu} in the  Appendix Section~\ref{moreExperiments} for a graphical view of  convergence in training. 
	%In fact, we solve the optimization problem in Equation~\eqref{ls} and Equation~\eqref{lsReLU} for~100 times, each time with a random initialization to obtain 100 estimators that are independent. 
	%Due to the non-convexity of the problem, it's highly probable that those estimators differ from each other.
	%For example, some of them might be saddle points,  local min, or global min. 
	%Then, we use the estimator with the smallest training error as a potential global optimum (due to the non-convexity of the objective function, global optimization is far reaching and so we call the trained network with the lowest training error just a 
	%potential global optimum), and the estimator with the highest training error as a stationary point
	%For ``relative error",  we use the error in potential global optimum (of the corresponding network) as the base.
	%\Res{And by ``relative error" we mean, dividing the error by a base, in this case, our base is the error for potential global optimum.}
	Results reveal that the test error for a potential global optimum and an approximate stationary point are very close in both linear and ReLU networks (relative errors for approximate stationary points are close to one for both linear and ReLU networks).
	Also note that the  reported numbers in Table~\ref{Tab-optim} are just relative errors to compare between training and test performance of a specific network so, 
	a comparison between the performance of linear and ReLU networks here is not meaningful.
	
	
	
	These observations reveal that: First, global optimization for neural networks is far reaching even for very simple neural networks. 
	Second, very practical outputs in deep learning (approximate stationary points) can still generalize  well---for linear networks and beyond.  We provide the similar result for a larger network in Table~\ref{Tab-optim-appen} and more detailed experiment explanations in   Appendix Section~\ref{moreExperiments}. 
	% even for ReLU neural  networks.   
	% \begin{center}
		%\begin{table}
		%\begin{tabular}{|l|ll|ll|}
		%\hline
		%  & \multicolumn{2}{c|}{Linear}  & \multicolumn{2}{c|}{ReLU}    \\ \hline
		%  & \multicolumn{1}{c|}{Optimization Error} & Test Error & \multicolumn{1}{c|}{Optimization Error} & Test Error \\ \hline
		%Potential Global Optima & \multicolumn{1}{c|}{0.72}   &   2.7468e-3 & \multicolumn{1}{c|}{1.04}   & 5.46e-2   \\ \hline
		%Potential Non-Global Optima & \multicolumn{1}{c|}{0.83}   &  2.7473e-3   & \multicolumn{1}{c|}{1.16}   &  5.96e-2  \\ \hline
		%\end{tabular}\caption{optimization error   vs. test error for trained  neural networks (with $\nbrinput=\nbrwidth=10$)  with   linear and ReLU  activations in a potential global optima and a potential non-global optima}
		%\label{Tab-optim}
		%\end{table}
		%\end{center}
		%\MH{Linear:  
			%Train: 0.79, 0.82, 0.68, 0.78, 0.79
			%Test: 2.74765, 2.74886, 2.748282,2.74856,2.74692e-3 (red, green, purple, blue, gray) and for ReLU networks: 
			%Train: 1.17,1.07,1.12,1.05,1.10 and Test error: 5.87,5.85,5.32,5,72,6.80e-2} 
		% These observations not only support our theories (in Section~\ref{Mainresult}), but also reinforce the traditional idea that theory of linear neural networks may  exhibit  also some properties of  complex networks. 
		% \begin{figure} 
			% 	\centering
			% 	\begin{subfigure}[t]{2.80in}
				% 		\centering
				% 		\includegraphics[width=7cm, height=5cm]{Figures/Test_Optim_Linear.png}
				% 		%\caption{linear and shallow neural network}
				% 	\end{subfigure}
			% 	\quad
			% 	\begin{subfigure}[t]{2.80in}
				% 		\centering
				% 		\includegraphics[width=7cm, height=5cm]{Figures/Test_Optim_Relu}
				% 		%\caption{ReLU and shallow neural network}
				% 	\end{subfigure}
			% 	\caption{Optimization error (colored curves)  for trained  neural networks (with $\nbrinput=\nbrwidth=10$)  with   linear (left panel) and ReLU (right panel) activations in $5$ different runs (allocated with different colors).   Due to the non-convexity of neural networks,  optimization algorithm may end up in different approximate stationary points.}
			% \end{figure}\label{fig:Optim_Linear&Relu}
		%\begin{figure} 
		%	\centering
		%	\begin{subfigure}[t]{2.5in}
			%		\centering
			%		\includegraphics[width=7cm, height=5cm]{Figures/Optim_Linear.png}
			%		\caption{ }
			%	\end{subfigure}
		%	\quad
		%	\begin{subfigure}[t]{2.5in}
			%		\centering
			%		\includegraphics[width=6.4cm, height=4.8cm]{Figures/Test_linear.png}
			% 		\caption{ }
			%	\end{subfigure}
		%		\begin{subfigure}[t]{2.5in}
			%		\centering
			%		\includegraphics[width=7cm, height=5cm]{Figures/Optim_Relu.png}
			%		\caption{ }
			%	\end{subfigure}
		%		\begin{subfigure}[t]{2.5in}
			%		\centering
			%		\includegraphics[width=7cm, height=5cm]{Figures/Test_Relu.png}
			%		\caption{ }
			%	\end{subfigure}
		%	\caption{Optimization error vs. test error  for trained  neural networks (with $\nbrinput=\nbrwidth=10$)  with   linear ((a) and (b)) and ReLU ((c) and (d)) activation functions  for $5$ different runs (allocated with different colors).   Due to the non-convexity of neural networks,  optimization algorithm may end up in different approximate stationary points, while the trained networks can still generalize  well.}
		%\end{figure}\label{fig:Optim_Linear&Relu}
		% \begin{figure}[]
			%     \centering
			%     \scalebox{1}{
				%     \includegraphics[width=7cm, height=5cm]{Figures/output_Optim_linear.png}
				%   }
			%     \scalebox{1}{
				%     \includegraphics[width=7cm, height=5cm]{Figures/output_Optim_Relu.png}}
			%     \caption{Test error (colored straight lines) vs. optimization error (colored curves) for  ($\ell_1$-)regularized least squares for shallow neural networks (with $\nbrinput=\nbrwidth=10$)  in 5 different runs (allocated with different colors) trained on  500  and tested on 300 data sample generated from a  standard normal distribution labeled by a sparse-target network (with the same structure as above) plus Gaussian noise.    Left panel shows the results for linear activations while the   right panel is for ReLU activations.   Due to the non-convexity of neural networks,  optimization algorithm  ends up in different approximate stationary points (a fixed  data set is employed for  5 different runs with different initializations), while the trained networks still generalize very well (straight lines are very close and even overlapped in most of the  cases).}
			%     \label{fig:Optim_Linear&Relu}
			% \end{figure}
		
		\begin{table}[h]
			\caption{Relative training error  and  test error for trained shallow neural networks (with $\nbrinput=10, \nbrwidth=10$)  with  linear and ReLU  activations in  a potential global optimum, an approximate stationary point, and a randomly generated network.}
			\label{Tab-optim}
			\begin{tabular}{lllll}
				\toprule
				& \multicolumn{2}{c}{Linear}                      & \multicolumn{2}{c}{ReLU}                        \\ 
				\cmidrule(r){2-3}\cmidrule(r){4-5}
				& \multicolumn{1}{c}{Training Error} & Test Error & \multicolumn{1}{c}{Training Error} & Test Error \\ %\hline
				Potential Global Optimum      & \multicolumn{1}{l}{\phantom{0000}1.000\phantom{0000}}              & \phantom{0000}1.000\phantom{000}         & \multicolumn{1}{l}{\phantom{000}1.000}              & 
				\phantom{000}1.000    \\ 
				Approximate Stationary Point & \multicolumn{1}{l}{\phantom{0000}1.001}           & \phantom{0000}1.001\phantom{}   & \multicolumn{1}{l}{\phantom{000}1.003}           & \phantom{000}1.004       \\ %\hline
				Randomly Generated  Network & \multicolumn{1}{l}{\phantom{}79618.240\phantom{0000}}          & 58198.240\phantom{000}   & \multicolumn{1}{l}{2120.060}           & {1980.060}      \\ 
				\bottomrule
			\end{tabular}
		\end{table}
		
		\section{Related literature}\label{RelatedWork}
		\input{Sections/Relatedworks}
		
		\section{Technical results}\label{TechResult}
		This section provides technical results needed for proving our main theories.  All the proofs as well as more related auxiliary results are deferred to  the Appendix. 
		\paragraph{Additional notations}\label{AddNotations}
		For  vectors
		$\ParamV=\vectorize(\parameterout,\parameterin)\in\R^{\EfDim}$ and $\boldsymbol{\alphaN}\deq(\alphaN_1,\dots,\alphaN_{\nbrwidth})\in\R^{\nbrwidth}$  with $\alphaN_{\jn}\ne 0$ for all $\jn\in\{1,\dots,\nbrwidth\}$, we 
		define $\ParamV_{\boldsymbol{\alphaN}}\deq\vectorize(\parameterout_{\boldsymbol{\alphaN}},\parameterin_{\boldsymbol{\alphaN}})\in\R^{\EfDim}$ as a rescaled version of $\ParamV$ with $(\parameterout_{\boldsymbol{\alphaN}})_{\jn}\deq\parameteroutj\cdot\alphaj$ and  $(\parameterin_{\boldsymbol{\alphaN}})_{\jn\kn}\deq\parameterinjk/\alphaj$ for all $\jn\in\{1,\dots,\nbrwidth\}$ and $\kn\in\{1,\dots,\nbrinput\}$.
		We tabulate the second order partial derivatives (subdifferentials) of $\objectiveFP{\parameterout,\parameterin}$ with respect to the $\ParamV=\vectorize(\parameterout,\parameterin)$ in a matrix called $\HessianF{\parameterout,\parameterin}\in \R^{\EfDim\times\EfDim}$.
		We use $\minevn[\cdot]$ to generate the smallest eigenvalue of a matrix.
		We use the notation $\boldsymbol{0}$ to generate a vector of zeros. 
		\subsection{Technical results for shallow linear neural networks}
		Here, we  provide technical results  that  are essential for proving our main theories for shallow linear networks but might also
		be of interest by themselves. 
		We first study the behavior of the Hessian matrix for shallow linear networks in a rescaled network as follows: 
		
		\begin{proposition}[Hessian Behavior for Shallow Linear Network]\label{PSDHessian}
			Suppose Assumption~\ref{assump} is verified 
			and  that $(\parameterout,\parameterin)\in\ParamSpaceM$ with 
			$\parameterin\parameterin\tp$ invertible. 
			Let $\GenVec\deq[(\GenVecSB)\tp,(\GenVecFB)\tp]\tp\in\R^{\EfDim}$ be a vector with $\normtwo{\GenVec}=1$, $\GenVecSB\in\R^{\nbrwidth}$, and $\GenVecFB\in\R^{\nbrwidth\cdot\nbrinput}$. 
			If $\GenVecSB= \boldsymbol{0}$ or $\GenVecFB= \boldsymbol{0}$,
			we have for all $\boldsymbol{\alphaN}\in\R^{\nbrwidth}\setminus\{\boldsymbol{0}\}$
			\begin{linenomath}
				\begin{equation*}
					\GenVec\tp\HessianF{\parameterout_{\boldsymbol{\alphaN}},\parameterin_{\boldsymbol{\alphaN}}}\GenVec~\ge~0\,;
				\end{equation*}
			\end{linenomath}
			Otherwise, above inequality holds for 
			all $\boldsymbol{\alphaN}\deq(1/\ConstC,\dots,1/\ConstC)\in\R^{\nbrwidth}$ with $\ConstC\in[1,\infty)$ such that
			\begin{linenomath}
				\begin{equation*}
					\ConstC^2 \ge \frac{2\normtwoB{\parameterout}^2\normtwoB{\GenVecFB}^2 +4\normtwoB{\GenVecSB}\normtwoB{\GenVecFB}\normtwoB{\parameterout\tp\parameterin-\parameteroutS\tp\parameterinS}}{\minevn\bigl[\parameterin\parameterin\tp\bigr]\normtwo{\GenVecSB}^2}\,.
				\end{equation*}
			\end{linenomath}
		\end{proposition}
		%The proof of Proposition~\ref{PSDHessian} is given in the  Appendix~\ref{proofs}.
		
		Note  that if $\GenVecSB= \boldsymbol{0}$ or $\GenVecFB= \boldsymbol{0}$, the quadratic product on the Hessian matrix (in a rescaled network with parameters $(\parameterout_{\Sc},\parameterin_{\Sc})$) is non-negative for all $\Sc$, otherwise, it is  non-negative just for $\Sc$ with large enough $\ConstC$.
		Proposition~\ref{PSDHessian} is employed for the proof of Theorem~\ref{OracleInSta}.
		
		
		\iffalse
		
		Result above  shows the behavior of Hessian matrix (population risk) in a scaled pair $(\parameterout_{\boldsymbol{\alphaN}},\parameterin_{\boldsymbol{\alphaN}})$ and reveals that for large enough $\ConstC$, which is the scaling parameter, the Hessian matrix is  ``approximately positive semidefinite".
		
		
		\fi
		
		\begin{lemma}[Empirical Processes]\label{EmpProcctwo}
			Under the Assumption~\ref{assump} 
			it holds for each  reasonable stationary  point $\ParamSta =\vectorize(\StaOut,\StaIn)$ of the objective function in~\eqref{ls} that 
			\begin{linenomath}
				\begin{equation*}
					\Bigl|\bigl(\DervSamSta-\DervPopSta\bigr)\tp(\ParamVS-\ParamSta)\Bigr|
					\le \tuningopt\normone{\ParamVS-\ParamSta}+\frac{\tuningopt}{2\nbrsamples}
				\end{equation*}
			\end{linenomath}
			with probability at least $1-1/{2\nbrsamples}$, where $\tuningopt$ is the oracle tuning parameter defined in~\eqref{oracletuning}. 
		\end{lemma}
		%The proof of Lemma~\ref{EmpProcctwo} is given in the  Appendix~\ref{proofs}.
		
		The result above establishes  a bound for the absolute difference between $\DervSamSta$ and $\DervPopSta$ for every reasonable stationary point  $(\StaOut,\StaIn)\in\ParamSpaceM$ for shallow linear  networks (a similar result can also be reached for shallow ReLU networks; see Remark~\ref{RemarkReLU}). 
		We employ Lemma~\ref{EmpProcctwo} choosing the optimal tuning parameter for the objective function~\eqref{ls}. 
		% Proposition~\ref{PSDHessian} and Lemma~\ref{EmpProcctwo} are the main ingredients for proving our Theorem~\ref{OracleInSta}.
		
		\input{Sections/technicalresults}
		
		
		
		
		%\section{More technical results}\label{MoreResult}
		%In this section, we establish five auxiliary results.
		%\subsection{More technical results}\label{MoreTechResult}
		%\input{Sections/technicalresults}
		%\subsection{Proofs}\label{proofs} 
		%\input{Sections/proofs}
		\section{Heavy-tailed noise}\label{Hnoise}
		\input{Sections/Heavy-Tail-The}
		%\section{High-level proof for Theorem~\ref{OracleInSta}}\label{App}
		%\input{Sections/Proof_The_1_high-level}
		\section{Discussion}\label{discussion}
		%	We have established statistical guarantees for approximate stationary points of regularized  shallow linear neural networks. 
		%	We have then extended our theories  to  shallow ReLU neural networks under mild assumptions  on the first layer weight matrix. 
		%	Despite being limited to shallow  networks,
		%	our theory is a large step forward in four ways:
		%	%First, previous empirical studies show that the optimization theory of linear-neural networks may exhibit some properties of non-linear models as well~\citep{saxe2013exact},
		%	%which means that our theories should also give some insights into non-linear networks (see also our Section~\ref{NumSec}).
		%	1.~Several papers consider the existence or non-existence of spurious local minima in linear neural networks under certain assumptions.
		%	Our theories work irrespective of whether there are local minima, and the theories also apply to saddle points, 
		%	which can also be hard to escape from in optimization.
		%	2.~Our extensions to ReLU neural networks not only justify why ReLU networks perform so well in practice but also support the common belief in the importance of effective initialization, such as near identity, in  the  optimization convergence~\citep{hardt2016identity}.
		%	3.~While  works like~\cite{bach2021gradient} consider convergence of specific optimization algorithms in deep learning, our results are agnostic to the optimization algorithm and, thus, much more general.
		%	%that 
		%	% the optimization theory of linear neural networks can exhibit some properties of non-linear models~\citep{saxe2013exact}.
		%	4.~And finally,
		%	our new statistical approach inspired by high-dimensional statistics is expected to spark further progress in the mathematical understanding of deep learning.
		We have established statistical guarantees for approximate stationary points of regularized  shallow linear neural networks. 
		We have then extended our theories  to  shallow ReLU neural networks under  the assumption  over  the first layer weight matrix. 
		Despite being limited to shallow  networks,
		our theory is a large step forward in four ways:
		1.~Several papers consider the existence or non-existence of critical points that are not global optima in linear neural networks under certain assumptions.
		In contrast, our theories apply regardless of whether such local minima or saddle points exist in the objective under consideration.
		2.~Our extensions to ReLU neural networks not only provide theoretical insights  but also highlight the importance of effective initialization, such as near-identity initialization, for ReLU networks~\citep{hardt2016identity}.
		3.~While  works like~\cite{bach2021gradient} consider convergence of specific optimization algorithms in deep learning, our results are agnostic to the optimization algorithm and do not require infinite-width networks, making our findings more general.
		4.~And finally, our new statistical approach inspired by high-dimensional statistics is expected to spark further progress in the mathematical understanding of deep learning.
		

